A Model Predictive Path Integral Method for Fast, Proactive, and Uncertainty-Aware UAV Planning in Cluttered Environments

Current motion planning approaches for autonomous mobile robots often assume that the low level controller of the system is able to track the planned motion with very high accuracy. In practice, however, tracking error can be affected by many factors, and could lead to potential collisions when the robot must traverse a cluttered environment. To address this problem, this paper proposes a novel receding-horizon motion planning approach based on Model Predictive Path Integral (MPPI) control theory -- a flexible sampling-based control technique that requires minimal assumptions on vehicle dynamics and cost functions. This flexibility is leveraged to propose a motion planning framework that also considers a data-informed risk function. Using the MPPI algorithm as a motion planner also reduces the number of samples required by the algorithm, relaxing the hardware requirements for implementation. The proposed approach is validated through trajectory generation for a quadrotor unmanned aerial vehicle (UAV), where fast motion increases trajectory tracking error and can lead to collisions with nearby obstacles. Simulations and hardware experiments demonstrate that the MPPI motion planner proactively adapts to the obstacles that the UAV must negotiate, slowing down when near obstacles and moving quickly when away from obstacles, resulting in a complete reduction of collisions while still producing lively motion.

==> model.tex <==
% % !TEX root = ICRA2020_runtime.tex

% \section{System Models} \label{sec:model}

% \NB{This section needs a better intro. Why are we using a quadrotor? We need to include this in the introduction too, i.e., we need to mention that in this work we apply the proposed scheme to quadrotor aerial vehicles motion planning case studies in cluttered environments under the effects of disturbances, however the proposed approach will apply to any autonomous vehicles}
% In this section, we explain the dynamical model of a quadrotor UAV, its controller, and the disturbance model considered in this work. We then explain the path planning algorithm.
% \NB{I would move this section (and shrink it) inside the method section, see comment inside the method section.}

% \subsection{Quadrotor UAV Dynamical Model}\label{sec:dynamics}
% A quadrotor can be modeled using the following  $12^\text{{th}}$ order state vector $\bm{x} = \begin{bmatrix} \bm{p}^T & \phi &\theta & \psi & \dot{\bm{p}}^T & \omega_x & \omega_y & \omega_z   \end{bmatrix}^{\mathsf{T}}$
% % \begin{equation*}
% % \bm{x} = \begin{bmatrix} x & y & z & v_x & v_y & v_z   \end{bmatrix}^{\mathsf{T}}
% % \end{equation*}
% where $\bm{p}^T = [ x, y, z ]$ and $\dot{\bm{p}}^T$ are the world frame positions and velocities, $\phi$, $\theta$, $\psi$ are the roll, pitch and yaw Euler angles and $\omega_x$, $\omega_y$, $\omega_z$ are the body frame angular velocities. The quadrotor dynamics can be defined as: $ \dot{\boldsymbol{x}} = f(\boldsymbol{x}, \boldsymbol{u}, \boldsymbol{d}) $ where $ \boldsymbol{u} =  \begin{bmatrix} F & \phi & \theta & \psi \end{bmatrix}^\mathsf{T} $ is the thrust, roll, pitch, and yaw inputs, and $ \boldsymbol{d} = \begin{bmatrix} d_x & d_y & d_z \end{bmatrix}^\mathsf{T}  $ is the external disturbance.
	
% The dynamics can be described as:


% \begin{align*}\label{eq:quadrotor_dynamics}
% \dot{\bm{p}}^{T} &= \begin{bmatrix}v_x & v_y & v_z\end{bmatrix}\\
% \begin{bmatrix}\dot{\phi} \\ \dot{\theta} \\ \dot{\psi}\end{bmatrix} &= \begin{bmatrix}1 & \sin\phi \tan\theta & \cos\phi \tan\theta\\ 0 & \cos\phi & -\sin\phi \\ 0 & \sin\phi \sec\theta & \cos\phi \sec\theta \end{bmatrix} \begin{bmatrix}\omega_{x} \\ \omega_{y} \\ \omega_{z} \end{bmatrix}\\
% \begin{bmatrix}\dot{v_x} \\ \dot{v_y} \\ \dot{v_z}\end{bmatrix} &= \begin{bmatrix}0 \\ 0 \\ -g \end{bmatrix} + \frac{1}{m} \begin{bmatrix}\cos\phi \cos\psi \sin\theta + \sin\phi \sin\psi \\ \cos\phi \sin\theta \sin\psi - \cos\psi \sin\phi \\ \cos\theta \cos\phi \end{bmatrix} u_1\\
% \begin{bmatrix}\dot{\omega_{x}} \\ \dot{\omega_{y}} \\ \dot{\omega_{z}}\end{bmatrix} &= \begin{bmatrix}\frac{I_{yy} - I_{zz}}{I_{xx}} \omega_{y}\omega_{z}\\ \frac{I_{zz} - I_{xx}}{I_{yy}} \omega_{x}\omega_{z} \\ \frac{I_{xx} - I_{yy}}{I_{zz}} \omega_{x}\omega_{y} \end{bmatrix} +  \begin{bmatrix}\frac{1}{I_{xx}} & 0 & 0\\ 0 & \frac{1}{I_{yy}} & 0\\ 0 & 0 & \frac{1}{I_{zz}}\end{bmatrix} \begin{bmatrix}u_{2} \\ u_{3} \\ u_{4} \end{bmatrix}
% \end{align*}

% where $ m $ is the mass of the quadrotor, $ g $ is gravity,and $I_{xx}$, $I_{yy}$,$ I_{zz}$ are diagonal inertial components.
% For linearization, we select a linearization point $(\bm{x}^*,u^*)$ when the system is at the hover state.


% \subsection{Controller Model}\label{sec:controller}
% \NB{this section can be cut down to a few sentences and included in the previous section with references to the iros 16 paper}
% In order to generate the roll, pitch and thrust inputs which make the system follow a desired trajectory or to reach a desired state, a cascaded set of PID controllers are used \cite{KumarRAM2010}. The inputs are generated as a function of the system state and the reference state on the trajectory: $ \boldsymbol{u} = g(\boldsymbol{x}, \boldsymbol{x}_{\tau}) $. Desired acceleration values are calculated using a position controller as follows:
% \begin{equation*} 
% 	\begin{aligned}
% 		& \ddot x_{des} = \ddot{x}_{\tau} + K_{p,x} (x_{\tau}-x) + K_{d,x} (\dot{x}_{\tau}-\dot{x}) \\
% 		& \ddot y_{des} = \ddot{y}_{\tau} + K_{p,y} (y_{\tau}-y) + K_{d,y} (\dot{y}_{\tau}-\dot{y}) \\
% 		& \ddot z_{des} = \ddot{z}_{\tau} + K_{p,z} (z_{\tau}-z) + K_{d,z} (\dot{z}_{\tau}-\dot{z}) \\	
% 	\end{aligned}		
% \end{equation*}
% where $ K_{p,x}, K_{p,y}, K_{p,z} $ are the proportional gains and $ K_{d,x}, K_{d,y}, K_{d,z} $ are the derivative gains of the position controller. $ x_{\tau}, y_{\tau}, z_{\tau} $ are the reference positions, $ \dot{x}_{\tau}, \dot{y}_{\tau}, \dot{z}_{\tau} $ are the reference velocities and $ \ddot{x}_{\tau}, \ddot{y}_{\tau}, \ddot{z}_{\tau} $ are the reference accelerations on the desired trajectory. Based on the dynamics of the system, the desired roll, pitch and thrust inputs to obtain desired acceleration values are calculated as follows:
% \begin{equation*}
% \begin{aligned}
% 	& \theta = (\ddot x_{des} \cos(\psi_{\tau}) +  \ddot y_{des} \sin(\psi_{\tau}))/g \\
% 	& \phi = (\ddot x_{des} \sin(\psi_{\tau}) +   \ddot y_{des} \cos(\psi_{\tau}))/g \\
% 	& F = m (\ddot z_{des} + g) \\
% \end{aligned}
% \end{equation*}
% where $ \psi_{\tau} $ is the reference yaw angle which is specified by the trajectory. 

%  \subsection{Disturbance Model}\label{sec:disturbance}
%  The external disturbance considered in this work is bounded in magnitude: $ \|\bm{d}\| \leq D_{max},  \forall~\bm{d} \in \mathcal D $ where $ D_{max} $ is the upper bound to the disturbance magnitude, and $ \mathcal{D} $ is the set of all possible disturbances. Here we assume that the online disturbance is unknown and can vary slowly over time. This is a reasonable assumption as wind disturbance generally follows a brownian motion and does not change erratically over short periods of time \cite{van2000statistics,palomaki2017wind}. 
%  %\EY{reference here}. 
%  % To capture the highest possible deviation during reachability analysis, we consider the disturbance with the highest possible magnitude in eight equidistant cardinal directions.
%  %of the UAV motion.
 
 
% \subsection{Trajectory Planning} \label{sec:traj}
%  To avoid collision with obstacles in the environment, we use a simple geometric approach for path planning. 
%  Specifically, For each obstacle in the environment, a waypoint is added to the path at a specified distance $ r_a $ if the distance between the current path to the goal and the obstacle is less than $ r_a $.
%  Then, a trajectory is generated to visit all the waypoints along the path by using a minimum jerk trajectory generation \cite{KumarRAM2010}.
 
%  It should be noted and highlighted that we present and use this path planning method due to its simplicity in implementation with simulators and experimental setup, however, the overall proposed framework is independent of the choice of path planning method. 
